Graphical House Allocation

The classical house allocation problem involves assigning $n$ houses (or items) to $n$ agents according to their preferences. A key criterion in such problems is satisfying some fairness constraints such as envy-freeness. We consider a generalization of this problem wherein the agents are placed along the vertices of a graph (corresponding to a social network), and each agent can only experience envy towards its neighbors. Our goal is to minimize the aggregate envy among the agents as a natural fairness objective, i.e., the sum of all pairwise envy values over all edges in a social graph. When agents have identical and evenly-spaced valuations, our problem reduces to the well-studied problem of linear arrangements. For identical valuations with possibly uneven spacing, we show a number of deep and surprising ways in which our setting is a departure from this classical problem. More broadly, we contribute several structural and computational results for various classes of graphs, including NP-hardness results for disjoint unions of paths, cycles, stars, or cliques, and fixed-parameter tractable (and, in some cases, polynomial-time) algorithms for paths, cycles, stars, cliques, and their disjoint unions. Additionally, a conceptual contribution of our work is the formulation of a structural property for disconnected graphs that we call separability which results in efficient parameterized algorithms for finding optimal allocations.

==> ack.tex <==
\begin{acks}
We would like to thank Andrew McGregor for pointing us to the linear arrangement problem, and for suggesting multiple useful lines of inquiry. The NP-hardness reduction from unary bin-packing was suggested by Cameron Musco. We would like to thank Yair Zick for help framing the problem. Funding?
\end{acks}

==> arxiv_00preamble.tex <==

% \usepackage{subcaption}

\usetikzlibrary{matrix,decorations.pathreplacing}

\usepackage{xcolor}

% If you use BibTeX in apalike style, activate the following line:
% \bibliographystyle{apalike}
\usepackage{easybmat}
\usepackage{multirow,bigdelim}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{paralist}
\let\Bbbk\relax
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage[justification = centering]{subcaption}
\usepackage{color}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{wrapfig,epsfig}
\usepackage{epstopdf}
\usepackage{url}
\usepackage{graphicx}
\usepackage{color}
\usepackage{epstopdf}
\usepackage[noend]{algpseudocode}
\usepackage{algorithmicx}
% \usepackage{scrextend}
\usepackage[T1]{fontenc}
\usepackage{bbm}
\usepackage{comment}
\usepackage{xspace}
\usepackage{thmtools}
%%% print refs in table of contents
\let\C\relax
\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{hyperref}  %%% arxiv don't allow this.
\hypersetup{colorlinks=true,citecolor=blue,linkcolor=blue} 
\usetikzlibrary{arrows}
%\usepackage[lmargin=1in,rmargin=1in,tmargin=0.8in,bmargin=0.8in]{geometry}
% \usepackage[margin=1in]{geometry}
% \linespread{1}
% %\newcommand{\QED}{\hfill$\qed$}
% % \graphicspath{{./figs/}}
% \newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
% \newcommand*{\centernot}{%
%   \mathpalette\@centernot
% }

\newenvironment{CompactItemize}{
\begin{list}{$\bullet$}{%
\setlength{\leftmargin}{12pt}
\setlength{\itemindent}{5pt}
\setlength{\topsep}{1pt}
\setlength{\itemsep}{-2pt}
}}
{\end{list}}

\newenvironment{CompactEnumerate}{
\begin{list}{\roman{enumi}.}{%
\usecounter{enumi}
\setlength{\leftmargin}{12pt}
\setlength{\itemindent}{5pt}
\setlength{\topsep}{1pt}
\setlength{\itemsep}{-2pt}
}}
{\end{list}}

\def\@centernot#1#2{%
  \mathrel{%
    \rlap{%
      \settowidth\dimen@{$\m@th#1{#2}$}%
      \kern.5\dimen@
      \settowidth\dimen@{$\m@th#1=$}%
      \kern-.5\dimen@
      $\m@th#1\not$%
    }%
    {#2}%
  }%
}



% \author{
% }



\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{open}[theorem]{Open Problem}
\newtheorem{question}[theorem]{Question}
\newtheorem{hypothesis}[theorem]{Hypothesis}


\newcommand{\pparagraph}[1]{\noindent \textbf{#1}}
% \newcommand{\tail}[2]{#1_{\overline{[#2]}}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\tabs}[1]{\left|#1\right|}
%\newcommand{\norm}[1]{\|#1\|}
%\newcommand{\inner}[1]{\langle#1\rangle}
\newcommand{\envy}{\textit{envy}}
\newcommand{\efxenvy}{\textit{strong-envy}}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\ov}{\overline}
\newcommand{\eps}{\epsilon}
\newcommand{\N}{\mathcal{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\volume}{\mathrm{volume}}
\newcommand{\RHS}{\mathrm{RHS}}
\newcommand{\LHS}{\mathrm{LHS}}
\renewcommand{\i}{\mathbf{i}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\varepsilon}{\epsilon}
\renewcommand{\tilde}{\wt}
\renewcommand{\hat}{\wh}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\DeclareMathOperator*{\E}{{\bf {E}}}
%\DeclareMathOperator*{\Pr}{{\bf{Pr}}}
\DeclareMathOperator*{\var}{\mathrm{Var}}
\DeclareMathOperator*{\Z}{\mathbb{Z}}
%\DeclareMathOperator*{\R}{\mathbb{R}}
%\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\C}{\mathbb{C}}
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\mean}{mean}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\nnz}{nnz}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\repeats}{repeat}
\DeclareMathOperator{\heavy}{heavy}
\DeclareMathOperator{\emp}{emp}
\DeclareMathOperator{\est}{est}
\DeclareMathOperator{\sparsity}{sparsity}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tucker}{tucker}
\DeclareMathOperator{\train}{train}
\DeclareMathOperator{\Diag}{diag}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\rect}{rect}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\Gram}{Gram}
\DeclareMathOperator{\Gaussian}{Gaussian}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Comb}{Comb}
\DeclareMathOperator{\signal}{signal}
% \DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\EMD}{EMD}
\DeclareMathOperator{\EEMD}{EEMD}
\DeclareMathOperator{\constraints}{constraints}
\DeclareMathOperator{\degree}{degree}
\DeclareMathOperator{\variables}{variables}
\DeclareMathOperator{\TV}{TV}
\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\cost}{cost}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\RAM}{RAM}
\DeclareMathOperator{\ati}{ati}
\DeclareMathOperator{\sym}{mon}
\DeclareMathOperator{\mon}{mon}
\DeclareMathOperator{\relu}{ReLU}
\DeclareMathOperator{\reg}{reg}
\DeclareMathOperator{\group}{group}
\newcommand{\Lat}{\mathcal{L}}
\newcommand{\SAT}{{\sf 3SAT}~}
\newcommand{\ESAT}{{\sf E3SAT}~}
\newcommand{\ESATB}{{\sf E3SAT(B)}~}
\newcommand{\MAX}{{\sf MAX}}
\newcommand{\BBB}{{\mathcal B}}
\newcommand{\AAA}{{\mathcal A}}
\newcommand{\DDD}{{\mathcal D}}
\newcommand{\MAXCUT}{{\sf MAX-CUT}~}
\newcommand{\CNF}{{\sf CNF}~}
\newcommand{\nCNF}{{\sf 3-CNF}~}
\newcommand{\kSUM}{{\sf k-SUM}~}
\newcommand{\kClique}{{\sf k-Clique}~}
\newcommand{\ETH}{{\sf ETH}~}
\newcommand{\NP}{{\bf{NP}}}
\newcommand{\RP}{{\bf{RP}}}
\newcommand{\EFXtwo}{{\textsf{EFX2} }}
% \renewcommand{\cal}[1]{\mathcal{#1}}


\definecolor{mygreen}{RGB}{80,180,0}
\definecolor{b2}{RGB}{51,153,255}
\definecolor{mycy2}{RGB}{255,51,255}


\newcommand{\COMMENT}[1]{\color{\blue} #1}
\newcommand{\Envy}{\mathsf{Envy}}


\colorlet{thechosenone}{red}
\colorlet{thechosentwo}{blue}
\makeatletter
\newcommand*{\RN}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother
\usepackage{lineno}
\def\linenumberfont{\normalfont\small}

\input{arxiv_libtheorems}

\newif\ifcomments
\commentstrue
\ifcomments
\newcommand{\rik}[1]{{\textcolor{red}{Rik: { #1}}}}
\else
\newcommand{\rik}[1]{}
\fi
\newif\ifcomments
\commentstrue
\ifcomments
\newcommand{\justin}[1]{{\textcolor{blue}{Justin: { #1}}}}
\else
\newcommand{\justin}[1]{}
\fi
\newif\ifcomments
\commentstrue
\ifcomments
\newcommand{\vignesh}[1]{{\textcolor{orange}{Vignesh: { #1}}}}
\else
\newcommand{\vignesh}[1]{}
\fi
\newif\ifcomments
\commentstrue
\ifcomments
\newcommand{\rohit}[1]{{\textcolor{magenta}{Rohit: { #1}}}}
\else
\newcommand{\rohit}[1]{}
\fi
\newif\ifcomments
\commentstrue
\ifcomments
\newcommand{\hadi}[1]{{\textcolor{purple}{Hadi: { #1}}}}
\else
\newcommand{\hadi}[1]{}
\fi
